SWIFT: A modern highly-parallel gravity and smoothed particle hydrodynamics solver for astrophysical and cosmological applications

Numerical simulations have become one of the key tools used by theorists in all the fields of astrophysics and cosmology. The development of modern tools that target the largest existing computing systems and exploit state-of-the-art numerical methods and algorithms is thus crucial. In this paper, we introduce the fully open-source highly-parallel, versatile, and modular coupled hydrodynamics, gravity, cosmology, and galaxy-formation code SWIFT. The software package exploits hybrid shared- and distributed-memory task-based parallelism, asynchronous communications, and domain-decomposition algorithms based on balancing the workload, rather than the data, to efficiently exploit modern high-performance computing cluster architectures. Gravity is solved for using a fast-multipole-method, optionally coupled to a particle mesh solver in Fourier space to handle periodic volumes. For gas evolution, multiple modern flavours of Smoothed Particle Hydrodynamics are implemented. SWIFT also evolves neutrinos using a state-of-the-art particle-based method. Two complementary networks of sub-grid models for galaxy formation as well as extensions to simulate planetary physics are also released as part of the code. An extensive set of output options, including snapshots, light-cones, power spectra, and a coupling to structure finders are also included. We describe the overall code architecture, summarise the consistency and accuracy tests that were performed, and demonstrate the excellent weak-scaling performance of the code using a representative cosmological hydrodynamical problem with $\approx$$300$ billion particles. The code is released to the community alongside extensive documentation for both users and developers, a large selection of example test problems, and a suite of tools to aid in the analysis of large simulations run with SWIFT.

==> cosmology/timesteps.tex <==
\subsection{Choice of time-step size}
\label{ssec:timesteps}

When running \swift with cosmological time-integration switched on, the
time-stepping algorithm gets modified in two ways. An additional criterion is
used to limit the maximal distance a particle can move and the integer time-line
used for the time-steps changes meaning and represents jumps in scale-factor
$a$, hence requiring an additional conversion.

\subsubsection{Maximal displacement}

to prevent particles from moving on trajectories that do not include the effects
of the expansion of the Universe, we compute a maximal time-step for the
particles based on their RMS peculiar motion and mean inter-particle separation:
\begin{equation}
  \Delta t_{\rm cosmo} \equiv \mathcal{C}_{\rm RMS} \frac{a^2}{\sqrt{\frac{1}{N_{\rm p}}\sum_i | \mathbf{v}_i' |^2}} d_{\rm p},
  \label{eq:dt_RMS}
\end{equation}
where the sum runs over all particles of a species $p$, $\mathcal{C}_{\rm RMS}$
is a free parameter, $N_{\rm p}$ is the number of baryonic or non-baryonic
particles, and $d_{\rm p}$ is the mean inter-particle separation at redshift $0$
for the particle with the lowest mass $m_i$ of a given species:
\begin{equation}
  d_{\rm baryons} \equiv \sqrt[3]{\frac{m_i}{\Omega_{\rm b} \rho_{\rm crit, 0}}}, \quad d_{\rm DM} \equiv \sqrt[3]{\frac{m_i}{\left(\Omega_{\rm m} - \Omega_{\rm b}\right) \rho_{\rm crit, 0}}}.
  \nonumber
\end{equation}
We typically use $\mathcal{C}_{\rm RMS} = 0.25$ and given the slow evolution of
this maximal time-step size, we only re-compute it every time the tree is
reconstructed.

We also apply an additional criterion based on the smoothing scale of the forces
computed from the top-level mesh.  In eq.~\ref{eq:dt_RMS}, we replace $d_{\rm
  p}$ by $a_{\rm smooth} \frac{L_{\rm box}}{N_{\rm mesh}}$, where we used the
definition of the mesh parameters introduced earlier. Given the rather coarse
mesh usually used in \swift, this time-step condition rarely dominates the
overall time-step size calculation.

\subsubsection{Conversion from time to integer time-line} 

\begin{equation}
  \int_{a_n}^{a_{n+1}} H dt = \int_{a_n}^{a_{n+1}} \frac{da}{a} =
  \log{a_{n+1}} - \log{a_n}.
\end{equation}


==> gravity/exact_forces.tex <==
\subsection{Exact forces for accuracy checks}
\label{ssec:exact_forces}

To assess the accuracy of the gravity solver, \swift can also compute
the gravitational forces and potential for a subset of particles using
a simple direct summation method. This is obviously much slower and
should only be used for code testing purposes. The forces for a
selection of particles are computed every time-step if they are active
and dumped to a file alongside the forces computed by the FMM method.

In the case where periodic boundary conditions are used, we apply the
\cite{Ewald1921} summation technique to include the contribution to
the forces of all the infinite periodic replications of the particle
distribution. We use the approximation to the infinite series of terms
proposed by \cite{Hernquist1991}\footnote{Note, however, that there is
  a typo in their formula for the force correction terms
  (eq. 2.14b). The correct expression is given by \cite{Klessen1997}
  \citep[see also][]{Hubber2011}.}, which we tabulate in one octant
using 64 equally spaced bins along each spatial direction spanning and
the range $[0,L]$, where $L$ is the side-length of the box.


==> sph/io/csds.tex <==
\subsection{Continuous non-blocking adaptive output strategy}
\label{ssec:io:csds}

In \swift we also include a novel output strategy called the \emph{Continuous
Simulation Data Stream} (CSDS), described by \cite{Hausammann2022}. The key
principles are summarised here \citep[for related ideas, see][]{Faber2010,
  Rein2017}.

In classic output strategies (\S\,\ref{ssec:io:snaps}), the simulation is
stopped at fixed time intervals and the current state of the system is written
to disk, similar to the frames of a movie. This is an expensive operation where
all the compute nodes suddenly stop processing the physics and instead put an
enormous stress on the communication network and file-system. During these
operations, the state of the system is not advanced, leading to an overall loss
in performance as the whole simulation has to wait until the i/o operations have
completed. Furthermore, in simulations with deep time-step hierarchies, only few
particles are active on most steps, with most particles just drifting
forward. In a cosmological context, a large fraction of the particles have
fairly simple trajectories, barely departing from \nth{1}- or \nth{2}-order
perturbation theory tracks. Only the small fraction of particles deep inside
haloes follow complex trajectories. For the first group of particles,
simulations typically have more snapshots than necessary to trace them, whilst
for the second group, even one thousand snapshots (say) over a Hubble time may
not be sufficient to accurately re-create their trajectory. It is hence natural
to consider a more adaptive approach.

The CSDS departs from the snapshot idea by instead creating a database of
updates. At the start of a simulation an entry is written for each particle. We
then start the simulation and progress the particles along. In its simplest
form, the CSDS then adds an entry for a particle to the database every few
($\sim10$) particle updates. As the writing is done on a particle-by-particle
basis, it can easily be embedded in the tasking system. Writing is no longer a
global operation where the whole simulation stops; rather updates are made
continuously. By writing an update every few particle steps, the trajectory of
each particle is, by construction, well-sampled, irrespective of whether it is
in a very active region (e.g. haloes) or not (e.g. in voids).  With this
mechanism, particles outside of structures can have as little as two entries
(start time and end time of the simulation) whilst some particles will have
thousands of entries. Since the time-step size of a particle is designed to
correctly evolve a particle, relying on this information to decide when to write
a database entry guarantees that the particles' evolution can later be
faithfully recreated.  Each entry for a particle contains a pointer to the
previous entry such that particles can easily be followed in time.

An improved version of this approach would be to write a database entry every
time a particle field has changed by some pre-defined fraction
$\varepsilon$. This is an important philosophical change; instead of creating
frames at fixed intervals, we can demand that the evolution of \emph{any}
quantity be reconstructed to some accuracy from the output and get the CSDS to
create the individual particle entries at the required times. The somewhat
arbitrary choice of time interval between snapshot is hence replaced by an
objective accuracy threshold.

This database of particle updates allows for many new simulation analysis
options. The trajectory and evolution of any particle can be reconstructed to
the desired accuracy; that is we have all the information for a high
time-resolution tracking of all the objects in a run. The first use is to
produce classic snapshots at any position in time. We simply interpolate all the
particle entries to that fixed time. But, one can also demand to construct
slices in space-time, i.e. a light-cone from the output. New possibilities
arising from this new output format will undoubtedly appear in the future. Tools
to perform the basic operations described here are part of the CSDS package
linked to \swift. The tools, and most of the analysis performed thus far, are
currently focused on dark-matter simulations, but we expect to extend this to
more complex scenarios in the future.





==> sph/io/ics.tex <==
\subsection{Initial Conditions}
\label{ssec:io:ics}

To ease the use of the code and given the large number of legacy initial
conditions (ICs) existing in the community using this format, we adopt the same
file format for input as the ``mode 3'' option of the \gadget-2 code
\citep{Springel2005}, i.e. the mode based on the \libraryname{hdf5} library
\citep{hdf5}.  \swift is fully compatible with any valid \gadget-2 set of
initial conditions, but we also provide additional optional features. Firstly,
we allow for different units to be used internally and in the ICs. \swift would
then perform a conversion upon start-up to the internal units. This can be
convenient when a certain set of ICs uses a range of values problematic when
represented in single-precision. Secondly, for cosmological runs, \swift can
also apply the necessary $h$-factor and $a$-factor corrections (see
\S\,\ref{ssec:ccordinates}) to convert to the system of co-moving coordinates
adopted internally.  A departure from the strict \gadget-2 format is that \swift
only allows for the data to be distributed over a single file; we do, however,
provide scripts to transform such distributed input files to our format.

Some tools also exist to directly generate \swift ICs with all the optional
features added. The \swiftsimio
\footnote{\url{https://github.com/SWIFTSIM/swiftsimio}} python package
\citep{swiftsimio} can be used to generate simple setups. The
\seagen \footnote{\url{https://github.com/jkeger/seagen}} \citep{Kegerreis2019}
and \woma\footnote{\url{https://github.com/srbonilla/WoMa}} \citep{RuizBonilla2021}
packages are designed to generate spherical or spinning planetary bodies in
equilibrium for collision problems (See sec. \ref{ssec:planetary}). For
cosmological simulations, the public version of the state-of-the-art ICs code
\monofonic%\footnote{\url{https://bitbucket.org/ohahn/monofonic/}}
\citep{Michaux2021,Hahn2021} has been extended to be able to produce files that
are directly compatible with the format expected by \swift. In particular,
information about the adopted cosmological parameters, phases, and all the
information required to re-generate the ICs are added to the files, read by
\swift, and propagated to the snapshots. This allows for runs to be reproduced
based solely on the information given in the \swift outputs.



==> sph/io/lightcones.tex <==
\subsection{Lightcone outputs}
\label{ssec:io:lightcones}

To bring the cosmological simulation outputs closer to observation mock
catalogs, \swift implements two separate mechanisms to record information as
particles cross the past light cone of a selection of observers placed in the
simulation box. The first mechanism writes the particles to disk as they reach a
distance from the observer corresponding to the light-travel distance of the
look-back time to the outputs. The second mechanism accumulates particle
information in redshift shells onto pixels to directly construct maps as the
simulation runs. See the Appendix of \cite{Schaye2022} for a detailed use case
of both these mechanisms.

\subsubsection{Particle data}

The position of each observer, the redshift range over which light-cone particle
output will be generated, and the opening angle of the cone are specified at run
time. At each time-step we compute the earliest and latest times that any
particles could be integrated forward to and the corresponding co-moving
distances. This defines a shell around each observer in which particles might
cross the past light cone as a result of drift operations carried out during
this time-step. An additional boundary layer is added to the inside of the shell
to account for particles that move during the time-step and assuming that they
have sub-luminal speeds.

For simulations employing periodic boundary conditions, we must additionally
output any periodic copy of a particle which crosses the observer's light
cone. We therefore generate a list of all periodic copies of the simulation
volume that overlap the shell around the observer. Then, whenever a particle is
moved, we check every periodic copy for a possible overlap with any of the
shells. If so, the particle's position is interpolated to the exact redshift at
which it crossed the lightcone and the particle is added to a writing
buffer. When the buffer reaches a pre-defined size, we write out the particles
including all their properties to disk.

To optimise the whole process, we take advantage of the way that \swift
internally arranges the particles in a cubic grid of cells
(\S\,\ref{ssec:parallel:cells}). We can use this structure to identify which
tree cells overlap with the current lightcone shells. This allows us to reduce
the number of periodic replications to check for every particle. Only the
particles in the cells previously identified need to undergo this process.

In most cases, the raw data generated by the particle lightcone requires some
post-processing; for instance to reorganise the particles inside the files in
terms of angular coordinates on the sky and redshift. 

\subsubsection{\healpix maps}

Light-cone particle outputs as well as the internal memory requirement rapidly
grow in size as the upper redshift limit is increased, especially if many box
replications occur, and can become impractical to store. \swift therefore also
contains a scheme to store spherical maps of arbitrary quantities on the light
cone with user specified opening angle, angular resolution, and redshift bins.

To this end, the observer's past light cone is split into a set of concentric
spherical shells in co-moving distance. For each shell we create one full-sky
\healpix \citep{Gorski2005} map for each quantity to be recorded. Whenever a
particle is found to have entered one of these shells, we accumulate the
particles' contributions to the \healpix maps for that shell. Typical examples
are the construction of mass or luminosity maps. Particles can also, optionally,
be smoothed onto the maps using an SPH kernel.

As the maps do not overlap in redshift, it is not necessary to store all of the
shells simultaneously in memory. Each map is only allocated and initialised when
the simulation first reaches the time corresponding to the outer edge of the
shell. It is then written to disk and its memory freed once all the particles
have been integrated to times past that corresponding to the light travel time
to the inner edge of the shell. In practice, the code will hence only need to
have a maximum of two maps in memory at any point in time.


==> sph/io/los.tex <==
\subsection{Line-Of-Sight outputs}
\label{ssec:los}

In addition to full-box snapshots, \swift can also produce so-called
\emph{line-of-sight} outputs. Randomly-positioned rays (typically perpendicular
to a face) are cast through the simulation volume and all gas particles whose
volumes are crossed by the infinitely thin rays are stored in a list. We then
write all the properties of these particles for each ray to a snapshot with a
format similar to the one described above but much reduced in volume. These
outputs can then be used to produce spectra via tools such as
\codename{SpecWizard} \citep{SpecWizard1,SpecWizard2}. Thanks to their small data
footprints, these line-of-sight snapshots are typically produced at high time
frequencies over the course of a run. This type of output is particularly
interesting for simulations of the IGM and Lyman-$\alpha$ forest (See
\S\,\ref{ssec:qla}).


==> sph/io/power_spectra.tex <==
\subsection{On-the-fly Power Spectra}
\label{ssec:io:ps}

Finally, \swift can compute a variety of auto- and cross- power
spectra at user-specified intervals. These include the mass density in
different particle species (and combinations thereof) as well as the
electron pressure. For the neutrino density, we also implement the
option to randomly select one half of the particles only or the
other. This helps reduce the shot-noise by computing a cross-spectrum
between the two halves.

The calculation is performed on a regular grid (usually of size $256^3$ and
hence allowing for the Fourier transform to be performed on a single node). 
Foldings \citep{Jenkins1998} are used to extend the range probed to smaller
scales with a typical folding factor of $4$ between iterations. Different window
functions from nearest-grid-point, to CIC, to triangular-shaped-clouds can be
used and are compensated for self-consistently \citep[see
e.g.][]{Colombi2009}. This could easily be extended to higher-order schemes and
to more particle properties.


==> sph/io/restart.tex <==
\subsection{Check-pointing mechanism}
\label{ssec:io:restart}

When running simulations at large computing centres, limits on the length of a
given compute job are often imposed. Many simulations will need to run for
longer than these limits and a mechanism to cleanly stop and resume a simulation
is thus needed. This \emph{check-pointing} mechanism can also be used to store
backups of the simulation's progress in case one needs to recover from a
software or hardware failure. Such a mechanism is different from the writing of
science-ready snapshots as all the information currently in the memory needs to
be saved; not just the interesting fields carried by the particles. These
outputs are thus typically much larger than the snapshots and are of the same
size as the memory used for the run.

In \swift, we choose to write one file per \techjargon{MPI} rank. No
pre-processing of any kind is done during writing. Each of the code's modules
writes its current memory state one after the other. This includes the raw
particle arrays, the cells, the tasks, and the content of the extensions (see
\S~\ref{sec:extensions}) among many other objects. At the start each module's
writing job we include a small header with some information about the size of
the data written. This allows us to verify that the data was read in properly
when resuming a simulation. As these are simple, unformatted, large, and
distributed writing operations, the code typically achieves close to the maximal
writing speed of the system. For the same \flamingo run mentioned above, the
whole procedure took $260~\rm{s}$ for 64 TB of data in $960$ files. This
corresponds to a raw writing speed of $250~\rm{GB/s}$. As the check-pointing is
fast, it is convenient to write files at regular intervals (e.g. every few
hours) to serve as a backup.

When restarting a simulation from a check-point file, the opposite operation is
performed. Each rank reads one file and restores the content of the memory. At
this point, the simulation is in exactly the same state as it was when the files
were written. The regular operations can thus resume as if no stoppage and
restarting operation had ever occurred.

As is the case in many software packages, our implementation is augmented with a
few practical options such as the ability to stop an on-going run or to ask the
simulation to run for a set wall-clock time before writing a check-point file
and stopping itself.




==> sph/io/snaps.tex <==
\subsection{Snapshots}
\label{ssec:io:snaps}

For the same convenience reasons as for the ICs, we also adopt an output file
format designed as a fully-compatible extension to the \gadget-2
\citep{Springel2005} ``mode 3'' format based on the \libraryname{hdf5} library
\citep{hdf5}.  We extend the format by creating new particle groups for the
species not existing in the original \gadget-2 code. We also add to the
snapshots a full copy of the parameters used to perform the simulation,
information about the version of the code, details of the cosmological models,
and information about the ICs. Another noteworthy extension is the extensive use
of units metadata in the snapshots. We attach full units information to every
field in the snapshots. That information includes human-friendly and
machine-readable conversion factors to the cgs system, as well as the conversion
factor needed to move between the co-moving and physical frame (See
sec. \ref{ssec:ccordinates}).  These metadata can be read by python packages
such as \swiftsimio \citep{swiftsimio} to then propagate this information
through the simulation analysis. This mechanism is based on the \libraryname{unyt}
\citep{unyt} library. The particles are stored in the snapshots in order of the
domain cells they belong to (See \S\,\ref{ssec:parallel:cells}).  Efficiently
retrieving the particles located in a small sub-region of the computational
domain is hence possible; for instance extracting the particles in the region
around a single halo only. In large simulations, this is much more efficient
than reading all the randomly ordered particles and then masking out the ones
that do not fall in the region of interest. Metadata to ease such reading
patterns are added to the snapshots. That information is picked up by tools such
as \swiftsimio to aid analysis of these massive simulations. The commonly used
visualisation package \libraryname{yt}\footnote{\url{https://yt-project.org/}} 
\citep{yt} has also been extended to directly read in \swift snapshots, including
the relevant meta-data.


The snapshots can either be written into one single file, with all nodes writing
collectively to the same dataset in parallel, or by splitting the data such that
each node writes a file with its local subset of particles. That second option
is preferable when using file systems that are not able to handle parallel
writes to a single file efficiently. When writing such a distributed snapshot,
an additional meta-snapshot is written; it contains all the information of a
regular single-file snapshot, but uses \libraryname{hdf5}'s virtual dataset
infrastructure to present the data distributed over many files as a single
contiguous array. The links between files are handled in the background by the
library. These meta-snapshots can then be read as if they were standard
snapshots, for instance via tools like
\libraryname{Gadgetviewer}\footnote{\url{https://github.com/jchelly/gadgetviewer/}}.
\swift can also optionally apply lossless compression to the snapshots (via
\libraryname{hdf5}'s own \libraryname{gzip} filter) as well as a per-field lossy
compression where the number of bits in the mantissa of the numbers can be
reduced to save disk space. This option is particularly interesting when
considering particle fields where the 23 bits of relative precision
(i.e. $\approx 7$ decimal digits) of a standard \techjargon{float} type are more
than sufficient for standard analysis\footnote{Classic examples are the
temperature field or the particles' metallicity.}. Similar filters can be
applied to \techjargon{double}-precision variables. Finally, \swift implements an
option to down-sample the particles of a given type in the snapshots by writing
only a fraction of the particles chosen at random.

As an example of i/o performance in a realistic scenario, the snapshots for the
recent flagship \flamingo run \citep{Schaye2022} were written in 200
seconds. They contain $2.65\times10^{11}$ particles of different types spread
over $960$ files totalling $39$ terabytes of data. This corresponds to a writing
speed of $200~\rm{GB}/\rm{s}$.  As this test only used 65\% of the systems'
nodes, this compares favourably to the raw capability ($350~\rm{GB}/\rm{s}$) of
the full cluster. Compressing the data using both lossy and lossless filters
reduces the snapshot size to $11$ terabytes but the writing time increases to
$1260$ seconds. This corresponds to a sustained writing speed of
$9~\rm{GB}/\rm{s}$; the difference is due to the compression algorithm embedded
within the \libraryname{hdf5} library. Additionally, by making use of the library's
parallel writing capability, we can repeat the uncompressed test but with all
nodes writing to a single file. In this configuration, we require $463$ seconds,
effectively achieving a sustained parallel writing speed of $86~\rm{GB}/\rm{s}$.

Snapshots can be written at regular intervals in time or change in scale-factor.
Alternatively, the user can provide a list of outputs in order to specify output
times more precisely. This list can be accompanied by a list of fields (or of
entire particle types) the user does not want to be written to a snapshot. This
allows for the production of reduced snapshots at high-frequency; for instance
to finely track black holes. Any of the structure finders (\S\,\ref{sec:stf})
can be run prior to the data being written to disk to include halo membership
information of the particles in the outputs.






